Separating Data via Block Invalidation Time Inference for Write Amplification Reduction in Log-Structured Storage

Log-structured storage has been widely deployed in various domains of storage systems, yet its garbage collection incurs write amplification (WA) due to the rewrites of live data. We show that there exists an optimal data placement scheme that minimizes WA using the future knowledge of block invalidation time (BIT) of each written block, yet it is infeasible to realize in practice. We propose a novel data placement algorithm for reducing WA, SepBIT, that aims to infer the BITs of written blocks from storage workloads and separately place the blocks into groups with similar estimated BITs. We show via both mathematical and production trace analyses that SepBIT effectively infers the BITs by leveraging the write skewness property in practical storage workloads. Trace analysis and prototype experiments show that SepBIT reduces WA and improves I/O throughput, respectively, compared with state-of-the-art data placement schemes. SepBIT is currently deployed to support the log-structured block storage management at Alibaba Cloud.

==> ideal.tex <==
\section{Ideal Data Placement}
\label{sec:optimal}

We begin with the description of a log-structured system in \S\ref{subsec:system}.
Then we propose an ideal data placement strategy that eliminates WA, i.e.,
achieves a WA of 1, in a log-structured system assuming the future knowledge of
block invalidation time is known in \S\ref{subsec:ideal_placement}. We point
out that to achieve such an ideal data placement, we have to assume there is a
unlimited number of open segments.  We then conclude by discussing the
feasibility to achieve efficient data placement after removing both assumptions
in \S\ref{subsec:assumptions}, which inspires our design.

